Synthesizing Datalog Programs Using Numerical Relaxation

The problem of learning logical rules from examples arises in diverse fields, including program synthesis, logic programming, and machine learning. Existing approaches either involve solving computationally difficult combinatorial problems, or performing parameter estimation in complex statistical models. In this paper, we present Difflog, a technique to extend the logic programming language Datalog to the continuous setting. By attaching real-valued weights to individual rules of a Datalog program, we naturally associate numerical values with individual conclusions of the program. Analogous to the strategy of numerical relaxation in optimization problems, we can now first determine the rule weights which cause the best agreement between the training labels and the induced values of output tuples, and subsequently recover the classical discrete-valued target program from the continuous optimum. We evaluate Difflog on a suite of 34 benchmark problems from recent literature in knowledge discovery, formal verification, and database query-by-example, and demonstrate significant improvements in learning complex programs with recursive rules, invented predicates, and relations of arbitrary arity.

==> experiment-effectiveness-table.tex <==
\begin{table}[t]
\caption{Benchmarks characteristics and performance of \Difflog{} compared to \alps.
\textbf{Rec} and \textbf{\#Rel} shows the programs that require recursive rules, and the number of relations.
\textbf{\#Rules} represents the number of expected (\textbf{Exp}) and candidate rules (\textbf{Cand}).
\textbf{\#Tuples} shows the number of input and output tuples.
\textbf{\#Iter} and \textbf{MCMC} report the number of iterations and MCMC samplings. \textbf{Time} shows the running time of \Difflog{} and \alps{} in seconds.
The timeout is set to one hour.}
\small
\begin{tabular}{l@{\ \ }lrrrrrrrrrrr}
\toprule
 &
\multirow{2}{*}{\textbf{Benchmark}} &
\multirow{2}{*}{\textbf{Rec}}&
\multirow{2}{*}{\textbf{\#Rel}} &
\multicolumn{2}{c}{\textbf{\#Rules}} &
\multicolumn{2}{c}{\textbf{\#Tuples}} &
\multicolumn{3}{c}{\Difflog{}} &
\multicolumn{1}{c}{\alps{}} \tabularnewline
\cmidrule(l{2pt}r{2pt}){5-6}\cmidrule(l{2pt}r{2pt}){7-8}\cmidrule(l{2pt}r{2pt}){9-11}\cmidrule(l{2pt}r{2pt}){12-12}
& & & & \textbf{Exp} & \textbf{Cand} & \textbf{In} & \textbf{Out} &
\textbf{\#Iter} & \textbf{MCMC} & \textbf{Time} &
\textbf{Time} \tabularnewline
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{\sf Knowelge Discovery}}	&	inflamation	&		&	7	&	2	&	67	&		&		&	3	&	0	&	1	&	2	&	\tabularnewline	
	&	abduce	&		&	4	&	3	&	38	&		&		&	1	&	0	&	$< 1$	&	2	&	\tabularnewline	
	&	animals	&		&	13	&	4	&	76	&		&		&	1	&	0	&	$< 1$	&	40	&	\tabularnewline	
	&	ancestor	&	\checkmark	&	4	&	4	&	38	&		&		&	1	&	0	&	$< 1$	&	14	&	\tabularnewline	
	&	buildWall	&	\checkmark	&	5	&	4	&	178	&		&		&	5	&	1	&	4	&	67	&	\tabularnewline	
	&	samegen	&	\checkmark	&	3	&	3	&	166	&		&		&	1	&	0	&	1	&	12	&	\tabularnewline	
	&	path	&	\checkmark	&	2	&	2	&	5	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	scc	&	\checkmark	&	3	&	3	&	166	&		&		&	6	&	1	&	4	&	56	&	\tabularnewline	\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{\sf Program Analysis}}	&	polysite	&		&	6	&	3	&	325	&		&		&	7	&	1	&	41	&	84	&	\tabularnewline	
	&	downcast	&		&	9	&	4	&	359	&		&		&	4	&	0	&	31	&	1,646	&	\tabularnewline	
	&	rv-check	&		&	5	&	5	&	67	&		&		&	4,506	&	151	&	57	&	195	&	\tabularnewline	
	&	andersen	&	\checkmark	&	5	&	4	&	140	&		&		&	3	&	1	&	26	&	27	&	\tabularnewline	
	&	1-call-site	&	\checkmark	&	9	&	4	&	96	&		&		&	5	&	1	&	7	&	106	&	\tabularnewline	
	&	2-call-site	&	\checkmark	&	9	&	4	&	103	&		&		&	29	&	1	&	143	&	676	&	\tabularnewline	
	&	1-object	&	\checkmark	&	11	&	4	&	41	&		&		&	3	&	1	&	4	&	345	&	\tabularnewline	
	&	1-type	&	\checkmark	&	12	&	4	&	39	&		&		&	4	&	0	&	5	&	13	&	\tabularnewline	
	&	1-obj-type	&	\checkmark	&	13	&	5	&		&		&		&	N/A	&	N/A	&	\textit{timeout}	&	\textit{timeout}	&	\tabularnewline	
	&	escape	&	\checkmark	&	10	&	6	&	29	&		&		&	5	&	1	&	1	&	5	&	\tabularnewline	
	&	modref	&	\checkmark	&	13	&	10	&	34	&		&		&	1	&	0	&	1	&	2,836	&	\tabularnewline	\midrule
\multirow{15}{*}{\rotatebox[origin=c]{90}{\sf Relational Queries}}	&	sql-01	&		&	≤ 7	&	≤ 4	&	26	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-02	&		&		&		&	12	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-03	&		&		&		&	1	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-04	&		&		&		&	5	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-05	&		&		&		&	1	&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-06	&		&		&		&		&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-07	&		&		&		&		&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-08	&		&		&		&		&		&		&	1	&	0	&	1	&	1	&	\tabularnewline	
	&	sql-09	&		&		&		&		&		&		&	2	&	1	&	1	&	$< 1$	&	\tabularnewline	
	&	sql-10	&		&		&		&		&		&		&	19	&	1	&	38	&	41	&	\tabularnewline	
	&	sql-11	&		&		&		&		&		&		&	9	&	1	&	1	&	1	&	\tabularnewline	
	&	sql-12	&		&		&		&		&		&		&	2	&	1	&	1	&	$< 1$	&	\tabularnewline	
	&	sql-13	&		&		&		&		&		&		&	1	&	0	&	$< 1$	&	$< 1$	&	\tabularnewline	
	&	sql-14	&		&		&		&		&		&		&	1	&	0	&	$< 1$	&	54	&	\tabularnewline	
	&	sql-15	&		&		&		&		&		&		&	N/A	&	N/A	&	\textit{timeout}	&	11	&	\tabularnewline	
\bottomrule
\end{tabular}
\label{tbl:benchmarks}
\end{table}

==> figs/mcmc-w-median.tex <==
\begin{table}[t!]\small\center
\caption{Effectiveness of MCMC  sampling in terms of the best running time (\textbf{Best}), median running time (\textbf{Median}) and the number of timeouts (\textbf{T/O}) out of 32 independent runs.}
\begin{tabular}{l@{\quad}rrr@{\quad}rrrrrr}
\toprule
\multirow{2}{*}{\textbf{Benchmark}} &
\multicolumn{3}{c@{\quad}}{\textbf{Hybrid}} &
\multicolumn{3}{c}{\textbf{Newton}}  &
\multicolumn{3}{c}{\textbf{MCMC}}
\tabularnewline
\cmidrule(l{0pt}r{10pt}){2-4}
\cmidrule(l{0pt}r{6pt}){5-7}
\cmidrule(l{6pt}r{6pt}){8-10}
& \textbf{Best} & \textbf{Median} & \textbf{T/O}
& \textbf{Best} & \textbf{Median} & \textbf{T/O}
& \textbf{Best} & \textbf{Median} & \textbf{T/O}  \tabularnewline\midrule
\texttt{polysite}	&	27s	& 142s &	0	&	10s	& 72s &	0	&	12s	& 76s &	0	\tabularnewline	
\texttt{downcast}	&	30s	& 310s &	2	&	16s	& 252s &	9	&	70s	& 268s &	7	\tabularnewline	
\texttt{rv-check}	&	22s	& 948s &	2	&	N/A	& N/A &	32	&	N/A	& N/A &	32	\tabularnewline	
\texttt{andersen}	&	4s	& 29s &	0	&	3s	& 15s &	10	&	4s	& 17s &	9	\tabularnewline	
\texttt{1-call-site}	&   4s	&  18s &	0	&	8s & 18s	&	1	&	N/A	& N/A &	32	\tabularnewline	
\texttt{2-call-site}	&	53s	& 225s &	0	&	27s	& N/A &	17	&	42s	& 94s &	9	\tabularnewline	
\texttt{1-object}	&	3s	&  17s &	0	&	3s	& N/A &	17	&	N/A	& N/A &	32	\tabularnewline	
\texttt{1-type}	&	4s	& 12s &	0	&	3s	& N/A &	18	&	N/A	& N/A &	32	\tabularnewline	
\texttt{escape}	&	1s	& 2s &	0	&	1s	& N/A &	17	&	N/A	& N/A &	32	\tabularnewline	
\texttt{modref}	&	1s	& 2s &	0	&	1s	& 1s &	4	&	N/A	& N/A &	32	\tabularnewline	\midrule
\textbf{Total}	&	&	&	4	& &		&	125	& &		&	217	\tabularnewline	
\bottomrule
\end{tabular}
\end{table}


==> shunt.tex <==
\section{Motivating Example}
\label{sec:Motivation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Introduce the example

Fundamentally, \Difflog{} is a system to learn Datalog programs from input-output examples. We illustrate our approach
in the context of synthesizing Andersen's pointer pointer analysis~\cite{andersen}, shown in Figure~%
\ref{fig:Motivation:Program}. This analysis statically reasons about the flow of information in pointer-manipulating
programs, and is central to a broad range of verification and compiler optimization tasks~\cite{smaragdakis:ftpl15}.

For instance, consider the C program of Figure~\ref{sfig:Motivation:Program:Code}. In this program, the pointer
\lstinline|b1| may point to (i.e., hold the address of) \lstinline|c1|, due to the statement \lstinline|b1 = &c1|. Other
examples of such points-to facts include \pointsTo(\lstinline|d|, \lstinline|f|). The design of fast and accurate
program analyses has been a challenge in the verification community: this paper considers the problem of automatically
synthesizing these analyses, using input-output data such as that shown in Figure~%
\ref{sfig:Motivation:Program:Analysis}.

\begin{figure*}
\begin{subfigure}[b]{0.3\textwidth}
  \lstinputlisting{figs/code.c}
  \caption{}
  \label{sfig:Motivation:Program:Code}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  \includegraphics[width=0.7\textwidth]{figs/pts_graph.pdf}
  \caption{}
  \label{sfig:Motivation:Program:Graph}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
  \centering \small
  \begin{tabular}{c} \toprule
  Input tuples (EDB) \\ \midrule
  \addrS(\texttt{b1}, \texttt{c1}) \\
  \loadS(\texttt{d}, \texttt{a1}) \\
  \storeS(\texttt{a1}, \texttt{d}) \\
  \copyS(\texttt{a2}, \texttt{a1}) \\
  $\cdots$ \\
  \bottomrule \end{tabular}
  \vspace{1em}

  \begin{tabular}{c} \toprule
  Output tuples (IDB) \\ \midrule
  \pointsTo(\texttt{a1}, \texttt{b1}) \\
  \pointsTo(\texttt{a1}, \texttt{b2}) \\
  \pointsTo(\texttt{a1}, \texttt{f}) \\
  \pointsTo(\texttt{a2}, \texttt{b1}) \\
  $\cdots$ \\
  \bottomrule \end{tabular}
  \caption{}
  \label{sfig:Motivation:Program:Relations}
\end{subfigure}
\vspace{1em}

\centering
\begin{subfigure}[b]{0.8\textwidth}
  \begin{tabular}{l} \toprule
  \strong{Input relations:} \addrS(\texttt{p}, \texttt{q}), \loadS(\texttt{p}, \texttt{q}),
                            \storeS(\texttt{p}, \texttt{q}), \copyS(\texttt{p}, \texttt{q}) \\
  \strong{Output relations:} \pointsTo(\texttt{p}, \texttt{q}) \\ \midrule
  $\begin{array}{lr@{\ }c@{\ }l}
    R_1: & \pointsTo(p, q) &\leads& \addrS(p, q). \\
    R_2: & \pointsTo(p, r) &\leads& \copyS(p, q), \pointsTo(q, r). \\
    R_3: & \pointsTo(p, s) &\leads& \loadS(p, q), \pointsTo(q, r), \pointsTo(r, s). \\
    R_4: & \pointsTo(r, s) &\leads& \storeS(p, q), \pointsTo(p, r), \pointsTo(q, s).
  \end{array}$ \\
  \bottomrule \end{tabular}
  \caption{}
  \label{sfig:Motivation:Program:Analysis}
\end{subfigure}
\caption{An example C program~(\ref{sfig:Motivation:Program:Code}) and its pointer
  graph~(\ref{sfig:Motivation:Program:Graph}). Figure~\ref{sfig:Motivation:Program:Relations} shows its representation
  as a set of relations. Designing fast and accurate pointer analyses has been a research challenge for the verification
  community, and we wish to automatically synthesize pointer analyses such as that in
  Figure~\ref{sfig:Motivation:Program:Analysis}.}
\label{fig:Motivation:Program}
\end{figure*}

%%%%
% 1a. Describe the synthesis goal

In the present example, the input data (also called the \emph{extensional} database or EDB) represents relevant facts
about the input C program, such as tuples \addrS($x$, $y$) for statements of the form \lstinline|$x$ = $y$|, tuples
\loadS($x$, $y$) for statements of the form \lstinline|$x$ = *$y$|, and so on. The output data (also called the
\emph{intentional} database or IDB) represents points-to facts, namely, tuples of the form \pointsTo($x$, $y$)
representing the proposition that $x$ may point to $y$. These tuples correspond to the solid edges of Figure~%
\ref{sfig:Motivation:Program:Graph}.

There are several challenges in learning program analyses in this manner. First, they include self-recursive and
mutually-recursive rules. For instance, rule $R_2$ states that if the program contains a statement $p = q$ and if we
have deduced that $q$ points to $r$, then we may deduce that $p$ points to $r$. Second, the rules follow patterns with
subtle variations, making it challenging to determine the space of candidate rules to consider. For instance, while the
rules $R_1$, $R_2$, and $R_3$ follow the ubiquitous \emph{chain pattern} whose general form is $r_0(x, y) \leads r_1(x,
t_1), r_2(t_1, t_2), \dots, r_n(t_{n - 1}, y)$, rule $R_4$ does not obey this pattern.

Many existing approaches do not support recursion, only support binary relations, and only
target rules that have a constrained form, such as the chain pattern.
In contrast, \Difflog\ supports recursive rules and relations of arbitrary arity.  Moreover, 
it generates a rich soup of candidate rules through a procedure called $k$-augmentation (see Sec.~\ref{sub:Framework:Learning}).
It starts out with the chain pattern and applies up to $k$ edits to generate increasingly rich variants;
when $k=\infty$, the soup contains all possible Datalog rules, although a small $k$ suffices in practice.
For instance, the pattern of rule $R_4$ is generated with $k=3$; the three edits correspond to the three
differences of $R_4$ compared to $R_3$.

Yet another challenge highlighted in the example is that, due to the undecidability of pointer analysis, no 
Datalog program can capture exact points-to facts for every C program.
In this case, we should still learn rules that best approximates the training data.
For instance, even though tuples {\small \pointsTo}({\tt b1}, {\tt c2}) and {\small \pointsTo}({\tt b2}, {\tt c1})
are excluded from the labeled output, we should learn the Andersen's analysis rules despite the fact that they
end up deriving those tuples.
This is possible only by leveraging continuous reasoning.
Existing approaches based on discrete reasoning fail to generate any rules in such cases.
Finally, the training data may contain noise in the form of mislabeled tuples; 
similarly, in such cases, we should learn rules that best explain the training data.

\Difflog\ satisfies all of the above criteria, and generates the depicted Datalog program in 500 iterations of
gradient descent in a total of 1.5 minutes.
In contrast, \nlp, which does not support recursion nor the non-chain pattern rule $R_4$, 
learns an approximate program that has 42.8\% RMS error even on the training data.
Finally, \metagol{}~\cite{metagol:ilp16} and \zaatar{}~\cite{Zaatar} are severely limited in their ability to scale in the presence of recursion and
increasing dataset size. As a result, \metagol{} times out on 7 of the benchmarks on which \Difflog{} successfully
learns the intended program.

